Provable Bounds for Learning Some Deep Representations

We give algorithms with provable guarantees that learn a class of deep nets in the generative model view popularized by Hinton and others. Our generative model is an $n$ node multilayer neural net that has degree at most $n^{\gamma}$ for some $\gamma <1$ and each edge has a random edge weight in $[-1,1]$. Our algorithm learns {\em almost all} networks in this class with polynomial running time. The sample complexity is quadratic or cubic depending upon the details of the model. The algorithm uses layerwise learning. It is based upon a novel idea of observing correlations among features and using these to infer the underlying edge structure via a global graph recovery procedure. The analysis of the algorithm reveals interesting structure of neural networks with random edge weights.

==> corrl-deep-pm.tex <==

%
%We now come to our main result, which is a multilayer version of the $0/\pm 1$ network we considered in Section~\ref{sec:3wise-pm}. We maintain the notation from the previous section, except that we have degree $2d_i$ in the graph at the $i$th layer (so that we have degree roughly $d_i$ each for $+1$ and $-1$ edges). 

%We will now combine ideas from the multilayer algorithm for $0/1$ weights and the analysis from \ref{sec:3wise-pm} to show that 3-wise correlations can be used to learn the network also in this case. We follow the same strategy as before: we will first learn the $+1$ weights in $G_1$. Then we use this information to decode the values of the hidden layer $h^{(2)}$ corresponding to our samples. Together with the strong unique neighbor property in $G_1$, we use this to find the support (more precisely, the non-edges) of the graph, which then gives the set of $-1$ edges.

%For the first part, 
%We prove the following, which requires a somewhat stronger assumption than before:

\begin{theorem}\label{thm:positive-edges:multi}
For any $1\le i\le \ell-1$, and if the network satisfies Property ?? with parameters $\rho_{i+1}^3 \ll \rho_{i}$, then given $O(\log n/\rho_{i+1}^2)$ samples, Algorithm~\ref{alg:3wise-corr} 3-WiseGraph constructs a hypergraph $\hat{G}$, where $(u,v,s)$ is an edge if and only if they share a positive neighbor in $G_i$. %Algorithm PairwiseGraph will recover the corresponding graph $\hat{G}$ in time $O()$ with high probability over the choice of samples. 

%If the parameter only satisfies $\rho_{i+1}^3 \ll \rho_{i}$, the 3-WiseGraph can be used to obtain the corresponding hypergraph $\hat{G}$ in time $O()$.
%Consider a deep network with layers $G_1, G_2, \dots, G_\ell$ and $\pm$ weights on the edges which satisfy the properties $\cP_{\pm}$. Suppose the $d_i$ and the density at the top layer $\rho_\ell$ satisfy the conditions \dots.

%Then the Algorithm~\textsf{3wise-correlations} finds the $+1$ edges in $G_1$ correctly with probability $\ge 1- n^{-C}$, for any constant $C$.
\end{theorem}
\iffalse
Let us recap the ideas we used to recover the $+1$ weights in Section~\ref{sec:single-pm}.  An output/hidden bit $h^{(i)}(u)$ will be $1$ iff the weighted sum of the neighbors in the previous level, i.e., 
\[ \sum_{v \in B_i(u)} w_{uv} h^{(i+1)}(v) >0. \]
Though the sum (as above) at each vertex has $d_i$ terms, typically there will only be at most one which is non-zero (since $u$ is typically a unique-neighbor of the set of non-zero vertices in $h^{(i+1)}$, which in turn is because of the range of $\rho_i$ we are operating in). Thus if we see an output $y_u =1$, it is, with reasonable probability, because of a single $+1$-parent activated in $h^{(1)}$. Thus if we look at the correlation $\Pr[ y_u=1 \wedge y_v=1 \wedge y_s=1 ]$ as above, it will be higher for $u,v,s$ with a common positive cause, which then allows us to identify the $+1$ edges in $G_1$.

Thus we want to estimate $\Pr[ y_u=1 \wedge y_v=1 \wedge y_s=1 ]$. As a warm-up, let us give upper and lower bounds for the probability $\Pr[y_u=1]$. We will denote by $\anc{i}_+(u)$ the vertices in $\anc{i}(u)$ which have an ``all $+1$'' path to $u$. For instance, $\anc{1}_+(u) = B_0^+ (u)$.

\begin{lemma}\label{lem:pm:warmup}
For any $u \in h^{(1)}$, we have
\begin{equation}\label{eq:pm:ub}
\Pr[y_u=1] \le \paren{1+ O(\log n) \cdot \sum_i d_i^{-1/2} } \rho_1
\end{equation}
\begin{equation}\label{eq:pm:lb}
\Pr[ y_u=1 ] \ge (9/10) \rho_1,
\end{equation}
\end{lemma}
\begin{proof}
\Tnote{Replace $y$ by $h^{(1)}$?}
The upper bound (Eq.~\eqref{eq:pm:ub}) is simple: we simply bound the probability by
$\Pr[ \anc{\ell}_+(u) \cap S \ne \emptyset]$, for which we can directly use the bounds in the previous section. (I.e., we ignore the effect of cancellations.)
\Tnote{Haven't gone through this proof...}
The lower bound is somewhat trickier. Here also, we will avoid cancellations, i.e., prove that we get $y_u=1$ with the desired probability, without cancellations at any level.
\[ \Pr[ y_u=1 ] \ge \Pr \left[ \paren{ \exists w\in B_0^+(u): ~h^{(1)}(w)=1 } \wedge \paren{ \forall w\in B_0^-(u): ~h^{(1)}(w)=0 } \right]. \]
We continue this for higher levels. At each level, there will be a {\em good} and {\em bad} set we maintain. Let us call them $\good^{(i)}(u)$ and $\bad^{(i)}(u)$ at level $i$. We maintain the invariant
\[ \Pr[ y_u=1 ] \ge \Pr\left[ \paren{ \exists w\in \good^{(i)}(u): h^{(i)}(w)=1 } \wedge \paren{ \forall w\in \bad^{(i)}(u): h^{(i)}(w)=0 } \right]. \]

We define these quantities iteratively. For $i=1$, we have $\good^{(i)}(u)= B_0^+(u)$ and $\bad^{(i)}(u)= B_0^-(u)$. Then, we define
\begin{align*}
\good^{(i+1)} &= B_i^+(\good^{(i)}) \setminus B_i^+(\bad^{(i)}) \\
\bad^{(i+1)} &= B_i^-(\good^{(i)}) \cup B_i^+(\bad^{(i)}) 
\end{align*}
Note that if at least one vertex of $\good^{(i+1)}$ is ``on'' and all the vertices in $\bad^{(i+1)}$ are off, then we must have the same for $i$. We can now bound the sizes of these sets using the expansion properties $\cP$. Let us denote $\epsilon:= (1/20\ell)$.
\begin{align*}
|\good^{(i+1)}| &\ge (1-\epsilon) \cdot d_{i+1} |\good^{(i)}| \\
|\good^{(i+1)}| &\le (1+ d_{i+1}^{-1/2}) \cdot d_{i+1} |\good^{(i)}| \\
|\bad^{(i+1)}| &\le (1+d_{i+1}^{-1/2}) \cdot \paren{d_{i+1} |\bad^{(i)}| +  d_{i+1} |\good^{(i)}| }
\end{align*}
A simple induction now shows that
\begin{align*}
|\good^{(i)}| &\ge (1-\epsilon)^i \cdot \frac{\rho_0}{\rho_i}, \\
|\bad^{(i)}| &\le (1+ d^{-1/2})^i \cdot (2i) \cdot \frac{\rho_0}{\rho_i}.
\end{align*}
Using these bounds with $i=\ell$, and applying the Lemma~\ref{lem:prob-calc3} completes the proof of the lemma.
\end{proof}
\fi

\begin{lemma}\label{lem:plusminus-deep}
Flor any $i\le \ell-1$ and any $u,v,s$ in the layer of $h^{(i)}$  ,  if they have a common positive neighbor(parent) in layer of $h^{(i+1)}$
\[ \Pr[h^{(i)}_u = h^{(i)}_v = h^{(i)}_s = 1] \ge \rho_{i+1}/3,\]
otherwise
\[ \Pr[h^{(i)}_u = h^{(i)}_v = h^{(i)}_s = 1] \le 2\rho_{i}^3 + 0.2\rho_{i+1}\]
%\text{ is } \begin{cases}{\ge ~~(9/10) \rho_2 \text{ ~if  $B_1^+(u)\cap B_1^+(v) \cap B_1^+(s) \ne \emptyset$,}}\\{
%		\le ~~ 2\rho_1^3 + 30\rho_2 \rho_1 + 10\rho_3 \text{~ otherwise.}} \end{cases} \]
\end{lemma}




%Note that the lower bound is weaker compared to Lemma~\ref{lem:3-wise-deep}, thus the distinguishing algorithm works only under slightly stronger assumptions than before. The lemma easily implies Theorem~\ref{thm:positive-edges:multi}, thus we turn to its proof
\Tnote{to define ``positive neighbor", to define $\rho_i = d_{i}\rho_{i+1}/2$}

\begin{proof}
Consider first  the case when $u,v$ and $s$ have a common positive  neighbor $z$ in the layer of $h^{(i+1)}$. Similar to the proof of Lemma~\ref{lem:3wise-single-pm}, when $h^{(i+1)}_z = 1$ and none of other neighbors of $u,v$ and $s$ in the layer of $h^{(i+1)}$ is fired, we know $h^{(i)}_u = h^{(i)}_v = h^{(i)}_s = 1$. However, since the distribution of $h^{(i+1)}$ is not uniformly sparse anymore, we cannot simply calculate the probability of this event.

In order to solve this problem, we go all the way back to the top layer. %, the distribution of which is uniform $\rho_{\ell}n_{\ell}$-sparse. 
Let $S = supp(h^{(\ell)})$, and let event $E_1$ be the event that $S\cap\anclp(u)\cap \anclp(v)\cap \anclp(s) \ne \emptyset$, and $S\cap (\ancl(u)\cup \ancl(v)\cup \ancl(s)) = S\cap\anclp(u)\cap \anclp(v)\cap \anclp(s)$ (that is, $S$ does not intersect at any other places except $\anclp(u)\cap \anclp(v)\cap \anclp(s)$). By the argument above we know $E_1$ implies $h^{(i)}_u = h^{(i)}_v = h^{(i)}_s = 1$.

%Thus $E_1$ implies that $h^{(i)}_u, h^{(i)}_v, h^{(i)}_s\textrm{ are all fired }$ because signals can only propagate to $u,v$ and $s$ via positive edges. 
Now we try to bound the probability of $E_1$.
Intuitively, $\anclp(u)\cap \anclp(v)\cap \anclp(s)$ contains $\anclp(z)$, which is of size roughly $d_{i+1}\dots d_{\ell-1}/2^{\ell-i-1} = \rho_{i+1}/\rho_{\ell}$. %because this is the number of positive ancestors of the common neighbor $z$.,  and 
On the other hand, $\ancl(u)\cup \ancl(v)\cup \ancl(s)$ is of size roughly $3d_{i}\dots d_{\ell-1} \approx 2^{\ell-i}\rho_{i}/\rho_{\ell}$. These numbers are still considerably smaller than $1/\rho_{\ell}$ due to our assumption on the sparsity of layers ($\rho_i \ll 1$). Thus by applying Lemma~\ref{lem:T1T2empty} with $T_1 = \anclp(z)$ and $T_2 = \ancl(u)\cup \ancl(v)\cup \ancl(s)$, we have
\[\Pr[h^{(i)}_u = h^{(i)}_v = h^{(i)}_s = 1]  \ge \Pr[S\cap T_1 \neq \emptyset, S\cap (T_2-T_1) = \emptyset] \ge \rho_{\ell}|T_1|/2 \ge \rho_{i+1}/3,\]
the last inequality comes from Property $\cPmul$. % that the graph is assumed to have. 

On the other hand, if $u,v$ and $s$ don't have a common positive neighbor in layer of $h^{(i+1)}$, consider event $E_2$: $S$ intersects each of $\anclp(u)$, $\anclp(v)$, $\anclp(s)$. Clearly, the target probability can be upperbounded by the probability of $E_2$. %by the probability of event $E_2$ that $S$ intersects each of $\ancl(u)$, $\ancl(v)$, $\ancl(s)$. 
By the graph properties we know each of the sets $\anclp(u),\anclp(v),\anclp(s)$ has size at most $A = 1.2d_{i}\dots d_{\ell-1}/2^{\ell-i}=1.2\rho_i/\rho_{\ell}$. Also, we can bound the size of their intersections by graph property $\cPmul$ and $\cPmulPlus$: $\card{\ancPO{\ell}(u)\cap \ancPO{\ell}(v)} \le B = 10\rho_{i+1}/\rho_{\ell}$, $\card{\anclp(u)\cap \anclp(v)\cap \anclp(s)} \le C = 0.1\rho_{i+1}/\rho_{\ell}$. Applying Lemma~\ref{lem:prob-calc2} with these bounds, we have
\[\Pr[E_2] \le \rho_{\ell}^3A^3 + 3\rho_{\ell}^2AB + \rho_{\ell}C \le 2\rho_{i}^3 + 0.2\rho_{i+1},\]
%
%
%, while they do have intersections with each other, so the probability of $E_2$ should be larger than simply $\rho^3|\ancl(u)||\ancl(v)||\ancl(s)| = \rho_{i}^3$. However, as long as the intersection of these three sets is reasonably bounded, as in the case when the graph is random, this term $\rho_i^3$ can be proved to be the dominating one. Formally, by Property $\cPmul$ and $\cPmulPlus$, we know that the size of  $\ancPO{\ell}(u)\cap \ancPO{\ell}(u)$ is bounded by $B = 10\rho_{i+1}'/\rho_{\ell}  = 102^{\ell-i}\rho_i/\rho_{\ell}$, and the size of  $\anclp(u)\cap \anclp(v)\cap \anclp(s)$ is bounded by $C = 0.1\rho_{i+1}/\rho_{\ell}$, since $u,v$ and $s$ don't have a common positive neighbor.  Plugging these into Lemma~\ref{lem:prob-calc2}, we have that when $\rho_i \ll 1$,
%\[\Pr[E_2] \le \rho_{\ell}^3A^3 + 3\rho_{\ell}^2AB + \rho_{\ell}C \le 2\rho_{i}^3 + 0.2\rho_{i+1},\]
%Hence the lemma is proved.
\end{proof}










%\begin{proof}
%The first inequality is proved along the lines of the proof of Lemma~\ref{lem:pm:warmup}. If $z$ is the common positive neighbor of $u,v,s$, we can set $\good^{(1)}=\{z\}$ and $\bad^{(1)}$ to be $B_1^-(u) \cup B_1^-(v) \cup B_1^-(s)$, and define $\good$, $\bad$ and $\epsilon$ inductively precisely as before. In this case, we have, for all $i\ge 1$,
%\begin{align*}
%|\good^{(i)}| &\ge (1-\epsilon)^{i-1} \cdot \frac{\rho_i}{\rho_1} \text{, and}\\
%|\bad^{(i)}| &\le (1+d^{-1/2})^i \cdot (6i) \cdot \frac{\rho_i}{\rho_0}.
%\end{align*}
%Now applying Lemma~\ref{lem:prob-calc3} gives the desired lower bound.
%
%The second is noting that $\Pr[ (S \cap \anc{\ell}_+(u) \ne \emptyset) \wedge (S \cap \anc{\ell}_+(u) \ne \emptyset) \wedge (S \cap \anc{\ell}_+(u) \ne \emptyset) ]$ is still an upper bound on $\Pr[ y_u=1 \wedge y_v=1 \wedge y_s=1]$ (this bound is very generous -- it ignores all potential cancellations). Thus using the upper bound from Lemma~\ref{lem:3-wise-deep} on the graph of $+1$ edges, we obtain the upper bound.
%\end{proof}
%
%This completes the proof of Lemma~\ref{lem:plusminus-deep}, and hence of Theorem~\ref{thm:positive-edges:multi}.







%\begin{lemma}\label{lem:deterministic_graph_property_pm}
%\begin{enumerate}
%\item $H^{i}_{+}(u) \approx 2^{-i}d_0\dots d_{i-1}$
%\end{enumerate}
%\end{lemma}





%\subsection{Reconstruction using pairwise correlations}
%
%Let us consider a graph with vertices placed in $c$ levels. The vertex sets in these levels are denoted by $V_1, \dots, V_c$, and write $|V_i| = n_i$. Suppose we have a random $d_i$ regular graph between vertex sets $V_i$ and $V_{i+1}$, for $1 \le i <c$. We denote this graph by $G_i$. 

%\subsubsection{The generating process}
%A set $S$ is formed by picking $k$ vertices u.a.r. from $V_1$, and we ``observe'' $Y(S) =\Gamma^{c-1}(S)$, i.e., the vertices in $V_c$ for which there is a length $(c-1)$ path from $S$. 
%
%The parameters $k, d_1, \dots, d_{c-1}$ are picked such that
%\[ k \cdot \prod_i d_i < n. \]
%We define densities $\rho_1, \dots, \rho_c$ by the equations $\rho_1 = k/n_1, \rho_2 = k d_1/n_2, \dots, \rho_c = k\prod_i d_i/n_c$. Thus in our setting, we have $\rho_1 < \rho_2 < \dots < \rho_c$.
%
%\subsubsection{The algorithm}
%For any two vertices $u,v$ in $V_c$, we would like to compute 
%\[ p^{(c)} (u,v) = \text{Prob}_S [ u, v \in Y ]. \]
%The hope is that for $u, v$ which have a common neighbor in $G_{c-1}$, the probability $p^{(c)}(u,v)$ is {\em slightly} higher than $u,v$ which do not have a common neighbor. If the difference is $\del>0$, then by observing $\otilde(1/\del^2)$ many samples $Y$, we can tell with good probability if $u, v$ have a common neighbor. This can then be used to reconstruct the graph.
%
%In computing the probability, we will have to use the fact that the $G_i$ are random bipartite graphs. However, we need to be careful since the graphs are first picked, and we {\em then} see many different samples $Y$. Assuming certain explicit conditions on the graphs $G_i$ we will prove bounds on $p^{(c)}(u,v)$. We then show that such conditions are satisfied w.h.p. when $G_i$ are all random bipartite graphs.
%
%Recall that $S$ contains each element of the first layer with probability precisely $\rho_1$. Denote by $\Gamma(u)$ the ``forward'' neighbors of $u$ (neighbors in the next level), and by $N(u)$ the back neighbors of $u$ (ones in the previous level). The `ancestors' of a vertex play a crucial role in the analysis. For $v \in V_c$, the ancestors are vertices in the set $N(v) \cup N^{(2)}(v) \cup \dots \cup N^{(c-1)}(v)$. %tree that is rooted at $v$. The trees consist of nodes $N(v), N^{(2)}(v), \dots, N^{(c-1)}(v)$. 
%
%We now state our main lemma. It will assume that the graphs $G_i$ satisfy certain explicit properties, needed in the proofs. For the moment, we avoid stating them formally, and simply denote them by $\calP$.
%
%[[@@@ The following probably changes if we have $n_i$ distinct. For now assume $n_i=n$ for all $i$.]]
%
%\begin{lemma}
%Suppose $G_1, \dots, G_{c-1}$ are graphs which satisfy $\calP$, and consider $u, v \in V_c$. If $N(u)$ and $N(v)$ are disjoint, then
%\begin{equation}\label{eq:corr-upper}
%\Pr[ Y_u =1 \wedge Y_v=1] \le \rho_c^2 + \rho_{c-1}/100.
%\end{equation}
%Otherwise (i.e., if $u$ and $v$ have a common back neighbor), we have
%\begin{equation}\label{eq:corr-lower}
%\Pr[ Y_u =1 \wedge Y_v=1] \ge \rho_c^2 + \rho_{c-1}/2.
%\end{equation}
%\end{lemma}
%
%Let us now outline the proof of the lemma. The first (eq.~\eqref{eq:corrupter}) is proved inductively. We can write out $\Pr[u \in Y \wedge v \in Y]$ as the probability that at least one of the vertices $N(u)$ and at least one of the vertices in $N(v)$ are in $\Gamma^{(c-2)}(S)$. This can then be written out as a sum of $d^2$ terms, ... [use induction, and the facwt that not too many pairs have a common neighbor in level $(c-2)$].
%
%Thus suppose now that 


%
%
%\begin{lemma}
%We could find some subset $T$ of size $C$ such that $T$ is a subset of some community in time ?? \Tnote{not sure, brute force gives time $n^C$, but I believe at least we could improve it to $(p^2mn)^C = (d_id_i')^C$. I think we may improve it to $n^3$ or even better.}
%\end{lemma}


%The following lemma says that basically the property we need is something like $|N^{(c-1)}(v)\cap N^{(c-1)}(u)| << d_1\cdots d_{c-2}$. 
%\begin{lemma}
%If the graph has the property that for every $u,v$ such that $N^{(1)}(u)\cap N^{(1)}(v) = \emptyset$, $|N^{(c-1)}(v)\cap N^{(c-1)}(u)| << d_1\cdots d_{c-2}$, and for every $u,v $ with $N^{(1)}(u)\cap N^{(1)}(v) \neq \emptyset$,$|N^{(c-1)}(v)\cap N^{(c-1)}(u)| \ge d_1\cdots d_{c-2}$,  then 
%\begin{enumerate}
%\item
% For $u,v$ with $N(u)\cap N(v) = \emptyset$, \[\Pr_{S}[u,v\in Y] \approx \rho_1|N^{(c-1)}(v)\cap N^{(c-1)}(u)| + \rho_1^2|N^{(c-1)}(v)|\cdot|N^{(c-1)}(u)| \le \rho_{c}^2 + \rho_1o(d_1\dots d_{c-2}),\]
%\item 
% For $u, v$ with $N(u)\cap N(v) \neq \emptyset$,  \[\Pr_S[u,v\in Y] \approx \rho_1|N^{(c-1)}(v)\cap N^{(c-1)}(u)| + \rho_1^2|N^{(c-1)}(v)|\cdot|N^{(c-1)}(u)| \ge  \rho_{c}^2 + \rho_1d_1\dots d_{c-2}\]
%\end{enumerate}
%\end{lemma}




%Lemma~\ref{lem:deterministic_graph_property} calculates $|H^{(i)}(u)\cap H^{(i)}(v)|$ inductively.
%\begin{lemma}[Informal]\label{lem:deterministic_graph_property}
%With probability $1-d^{-C}$, over the randomness of the graph, the followings hold: 
%
%\begin{enumerate}
%\item For every nodes $u\in Y$, and every $1\le i\le \ell$, $H^{(i)}(u) \approx d_{0}\dots d_{i-1}$
%\item For every pair of nodes $u,v \in Y$, and every $1\le i\le \ell $, $|H^{(i)}(u)\cap H^{(i)}(v)| \approx d_{i-1}|H^{(i-1)}(u)\cap H^{(i-1)}(v)| + \max\{d_{i-1}^2|H^{(i-1)}(u)|\cdot|H^{(i-1)}(v)|/n_{i}, 1\}$
%\item For every pair of nodes $u,v \in Y$, 
%\begin{eqnarray*}
%|N^{\ell}(u)\cap N^{\ell}(v)| &\approx& \max\{d_{\ell-1}^2|H^{(\ell-1)}(u)|\cdot|H^{(\ell-1)}(v)|/n_{\ell}, 1\} \\ && +d_{\ell-1}\max\{d_{\ell-2}^2|H^{(\ell-2)}(u)|\cdot|H^{(\ell-2)}(v)|/n_{\ell-1}, 1\} \\ && + \cdots + d_{\ell-1}\cdots d_{2}\max\{d_{1}^2|H^{(1)}(u)|\cdot|H^{(1)}(v)|/n_{2}, 1\} +\\
%&&+ d_{\ell-1}\cdots d_{2}d_{1}|H^{(1)}(u)\cap H^{(1)}(v)|
%\end{eqnarray*}
%\end{enumerate}
%\end{lemma}

%
%\begin{proof}[Proof Sketch]
%1 and 2 follows the expander property of the random graph. 3 can be obtained by using 1 and 2 inductively.
%\end{proof}
%
%The following two lemmas follow the 3 of Lemma~\ref{lem:deterministic_graph_property}
%
%\begin{lemma}\label{lem:gap_between_two_cases}
%With probability $1-d^{-C}$ over the randomness of the graph, 
%\begin{enumerate}
%\item if $|H^{(1)}(u)\cap H^{(1)}(v)| \ge 1$, then \[|H^{\ell}(v)\cap H^{\ell}(u)| \ge d_1\dots d_{\ell-1}\]
%\item if $H^{(1)}(u)\cap H^{(1)}(v) = \emptyset$, then  
%\begin{eqnarray*}
%|H^{\ell}(v)\cap H^{\ell}(u)| &\le & d_{\ell-1} \cdots d_{3}\max \{d_{1}^2d_{0}^2/n_{2}, 1\}  +  d_{\ell-1}\cdots d_{4}\max \{d_{2}^2d_{1}^2d_{0}^2/n_{3}, 1\} \\
%&& + \dots + \max \{d_{\ell-1}^2\dots d_{1}^2d_{0}^2/n_{\ell}, 1\} \end{eqnarray*}
%
%\end{enumerate}
%\end{lemma}
%

%
%
%
%\begin{lemma}
%\Tnote{Need modification}
%If $\rho_0 d_0= o(k)$, and $d_{i} = \omega(\log n)$, then with probability $1-d^{-C}$ over the randomness of the graph, for every pair $u,v$ with $H(u) \cap H(v) = \emptyset$, $|H^{\ell}(v)\cap H^{\ell}(u)| << d_1\cdots d_{\ell-1}$. 
%\end{lemma}

